A Generative Approach Towards Improved Robotic Detection of Marine Litter

This paper presents an approach to address data scarcity problems in underwater image datasets for visual detection of marine debris. The proposed approach relies on a two-stage variational autoencoder (VAE) and a binary classifier to evaluate the generated imagery for quality and realism. From the images generated by the two-stage VAE, the binary classifier selects "good quality" images and augments the given dataset with them. Lastly, a multi-class classifier is used to evaluate the impact of the augmentation process by measuring the accuracy of an object detector trained on combinations of real and generated trash images. Our results show that the classifier trained with the augmented data outperforms the one trained only with the real data. This approach will not only be valid for the underwater trash classification problem presented in this paper, but it will also be useful for any data-dependent task for which collecting more images is challenging or infeasible.

==> results/binary.tex <==
\begin{table}[t]
\setlength\belowcaptionskip{-0pt}
\centering
    \caption{Binary classifier evaluation}
  \begin{tabular}{p{1cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}}
     & Training Acc. & Validation Acc. & Test Acc. \\ \hline
     Bag & 0.89 & 0.88 & 0.86 \\ \hline
     Bottle & 0.88 & 0.83 & 0.82 \\
  \end{tabular}
    \label{tb:binary}
    \vspace{-0mm}
\end{table}


==> results/classifier.tex <==
\begin{table}[H]
\setlength\belowcaptionskip{-0pt}
\centering
    \caption{A multi-class classifier architecture}
  \begin{tabular}{p{2cm}|p{2cm}}
  Layer & Shape \\ \hline
  Input & $ 128 \times 128 \times 3$ \\
    Reshape & $ 32 \times 32 \times 3$ \\
    Conv & $ 29 \times 29 \times 32$ \\
    Max-Pooling & $ 28 \times 28 \times 32$ \\
    Conv & $ 26 \times 26 \times 64$ \\
    Max-Pooling &$ 25 \times 25 \times 64$ \\
    Flatten & $40000 \times 1 $ \\
    Dense & $100 \times 1 $ \\
    Dropout & $100 \times 1$ \\
    Output & $3 \times 1$ \\
  \end{tabular}
    \label{tb:classifier}
    \vspace{-0mm}
\end{table}


==> results/fidtable.tex <==
\begin{table}[H]
\setlength\belowcaptionskip{-0pt}
\centering
    \caption{FID scores for each class}
  \begin{tabular}{p{1cm}|p{1cm}|p{1cm}|p{1cm}}
     & Stage 1 & Stage 2 & Reconst. \\ \hline
     Bag & 98 & 196 & 175 \\ \hline
     Bottle & 223 & 301 & 240 \\
  \end{tabular}
    \label{tb:fid}
    \vspace{-0mm}
\end{table}


==> results/plasticbag.tex <==
\begin{figure*}[t!]
\setlength{\lineskip}{0pt}
\centering
\setlength\tabcolsep{1.pt}
\renewcommand{\arraystretch}{0.5}
  \begin{tabular}{cccccccccc}
  \raisebox{1.\normalbaselineskip}[0pt][0pt]{\multirow{3}{*}{\rotatebox[origin=c]{90}{Plastic Bag}}} &
  \raisebox{2.\normalbaselineskip}[0pt][0pt]{\rotatebox[origin=c]{90}{Stage 1}} &
    \includegraphics[width=.11\textwidth]{results/gen1_sample10.png} &
    \includegraphics[width=.11\textwidth]{results/gen1_sample11.png} &
    \includegraphics[width=.11\textwidth]{results/gen1_sample12.png} &
    \includegraphics[width=.11\textwidth]{results/gen1_sample13.png} &
    \includegraphics[width=.11\textwidth]{results/gen1_sample15.png} &
    \includegraphics[width=.11\textwidth]{results/gen1_sample16.png} &
    \includegraphics[width=.11\textwidth]{results/gen1_sample17.png} &
    \includegraphics[width=.11\textwidth]{results/gen1_sample18.png}   \\
    &
  \raisebox{2.\normalbaselineskip}[0pt][0pt]{\rotatebox[origin=c]{90}{Stage 2}} &
    \includegraphics[width=.11\textwidth]{results/gen2_sample84.png} &
    \includegraphics[width=.11\textwidth]{results/gen2_sample111.png} &
    \includegraphics[width=.11\textwidth]{results/gen2_sample155.png} &
    \includegraphics[width=.11\textwidth]{results/gen2_sample177.png} &
    \includegraphics[width=.11\textwidth]{results/gen2_sample304.png} &
    \includegraphics[width=.11\textwidth]{results/gen2_sample330.png} &
    \includegraphics[width=.11\textwidth]{results/gen2_sample376.png} &
    \includegraphics[width=.11\textwidth]{results/gen2_sample452.png}   \\
    
    &      \raisebox{2.\normalbaselineskip}[0pt][0pt]{\rotatebox[origin=c]{90}{Reconst.}} &
    \includegraphics[width=.11\textwidth]{results/recon_sample1.png} &
    \includegraphics[width=.11\textwidth]{results/recon_sample2.png} &
    \includegraphics[width=.11\textwidth]{results/recon_sample3.png} &
    \includegraphics[width=.11\textwidth]{results/recon_sample4.png} &
    \includegraphics[width=.11\textwidth]{results/recon_sample6.png} &
    \includegraphics[width=.11\textwidth]{results/recon_sample7.png} &
    \includegraphics[width=.11\textwidth]{results/recon_sample8.png} &
    \includegraphics[width=.11\textwidth]{results/recon_sample73.png}   \\
    
  \raisebox{1.\normalbaselineskip}[0pt][0pt]{\multirow{3}{*}{\rotatebox[origin=c]{90}{Plastic Bottle}}} &
\raisebox{2.\normalbaselineskip}[0pt][0pt]{\rotatebox[origin=c]{90}{Stage 1}} &
    \includegraphics[width=.11\textwidth]{results_bottle/gen1_sample0.png} &
    \includegraphics[width=.11\textwidth]{results_bottle/gen1_sample1.png} &
    \includegraphics[width=.11\textwidth]{results_bottle/gen1_sample2.png} &
    \includegraphics[width=.11\textwidth]{results_bottle/gen1_sample3.png} &
    \includegraphics[width=.11\textwidth]{results_bottle/gen1_sample4.png} &
    \includegraphics[width=.11\textwidth]{results_bottle/gen1_sample5.png} &
    \includegraphics[width=.11\textwidth]{results_bottle/gen1_sample6.png} &
    \includegraphics[width=.11\textwidth]{results_bottle/gen1_sample7.png}   \\
    &
\raisebox{2.\normalbaselineskip}[0pt][0pt]{\rotatebox[origin=c]{90}{Stage 2}} &
    \includegraphics[width=.11\textwidth]{results_bottle/gen2_sample8.png} &
    \includegraphics[width=.11\textwidth]{results_bottle/gen2_sample19.png} &
    \includegraphics[width=.11\textwidth]{results_bottle/gen2_sample26.png} &
    \includegraphics[width=.11\textwidth]{results_bottle/gen2_sample91.png} &
    \includegraphics[width=.11\textwidth]{results_bottle/gen2_sample94.png} &
    \includegraphics[width=.11\textwidth]{results_bottle/gen2_sample133.png} &
    \includegraphics[width=.11\textwidth]{results_bottle/gen2_sample187.png} &
    \includegraphics[width=.11\textwidth]{results_bottle/gen2_sample207.png}   \\
    
    &  \raisebox{2.\normalbaselineskip}[0pt][0pt]{\rotatebox[origin=c]{90}{Reconst.}} &
    \includegraphics[width=.11\textwidth]{results_bottle/recon_sample76.png} &
    \includegraphics[width=.11\textwidth]{results_bottle/recon_sample78.png} &
    \includegraphics[width=.11\textwidth]{results_bottle/recon_sample81.png} &
    \includegraphics[width=.11\textwidth]{results_bottle/recon_sample83.png} &
    \includegraphics[width=.11\textwidth]{results_bottle/recon_sample85.png} &
    \includegraphics[width=.11\textwidth]{results_bottle/recon_sample86.png} &
    \includegraphics[width=.11\textwidth]{results_bottle/recon_sample87.png} &
    \includegraphics[width=.11\textwidth]{results_bottle/recon_sample95.png} \\
  \end{tabular}
  \caption{The images are samples of  the underwater two-stage VAE for each trash class}
  \label{fig:plasticbag}
\end{figure*}

% \begin{figure*}[htb]
% \setlength{\lineskip}{0pt}
% \centering
%     \text{hi}
%     \includegraphics[width=.12\textwidth]{example-image-a}%
%     \includegraphics[width=.12\textwidth]{example-image-b}%
%     \includegraphics[width=.12\textwidth]{example-image-c}%
%     \includegraphics[width=.12\textwidth]{example-image-a}%
%     \includegraphics[width=.12\textwidth]{example-image-b}%
%     \includegraphics[width=.12\textwidth]{example-image-c}%
%     \includegraphics[width=.12\textwidth]{example-image-c}%
%     \includegraphics[width=.12\textwidth]{example-image}\\
%     \includegraphics[width=.12\textwidth]{example-image-a}%
%     \includegraphics[width=.12\textwidth]{example-image-b}%
%     \includegraphics[width=.12\textwidth]{example-image-c}%
%     \includegraphics[width=.12\textwidth]{example-image-a}%
%     \includegraphics[width=.12\textwidth]{example-image-b}%
%     \includegraphics[width=.12\textwidth]{example-image-c}%
%     \includegraphics[width=.12\textwidth]{example-image-c}%
%     \includegraphics[width=.12\textwidth]{example-image}\\
%   \label{fig:plasticbag}
%   \caption{This is   some figure side by side}
% \end{figure*}





    %   \raisebox{2.\normalbaselineskip}[0pt][0pt]{\rotatebox[origin=c]{90}{Stage 2}} &
    % \includegraphics[width=.11\textwidth]{} &
    % \includegraphics[width=.11\textwidth]{} &
    % \includegraphics[width=.11\textwidth]{} &
    % \includegraphics[width=.11\textwidth]{} &
    % \includegraphics[width=.11\textwidth]{} &
    % \includegraphics[width=.11\textwidth]{} &
    % \includegraphics[width=.11\textwidth]{} &
    % \includegraphics[width=.11\textwidth]{} &   \\

==> tex/3_problem.tex <==
\section{Problem Formulation}
\label{sec:problem_formulation}


==> tex/todo.tex <==
\section{TODO}
\todo[inline, color=green!30]{Done}
\todo[inline, color=red!30]{Todo}
\todo[inline, color=orange!30]{Discard}
\begin{enumerate}
    \item \todo[inline, color=green!30]{Some typos or bad sentences are presented along the text.
For example:
-	“ … development of late, primarily …”
-	To estimate the the position …”}
    \item \todo[inline, color=orange!30]{Just a comparison between four
state-of-the-art and well-known/tested Bayes filters}
    \item \todo[inline, color=green!30]{Very difficult to understand what was done
in the experimental tests – how do you get the
depth/altitude data?;}
    \item \todo[inline, color=green!30]{ the algorithms presented (EKF/UKF/PF/MPF) are not
novel, nor is their application to AUV navigation using
bathymetric data. Consider rephrasing the abstract
to highlight the comparative/evaluative nature of the
contribution} \label{todoabs}
    \item \todo[inline, color=green!30]{Intro:  par. 1: landmarks can be detected by exteroceptive
sensors (e.g. side-scan sonar for passive landmarks,
{L,US}BL for active landmarks}\label{intropar1}
    \item \todo[inline, color=green!30]{Intro: par. 3: it could perhaps be clearer to say that it is
the altitude that varies with depth (for the same
location), hence the need for a depth sensor. The authors
could consider making their assumptions on available
measurements (e.g. depth and altitude) and what variables
are going to be estimated. At this point in the text, the
goal appears to be estimation of the full 6DoF
state, but the rest of the paper presents the state vector
as 3D position. Assuming accurate orientation (heading in
particular) often necessitates the use of highly accurate
IMU/INSs, or dedicated infrastructure. }\label{intropar3}
    \item \todo[inline, color=green!30]{Intro:  par. 5 (contribution): it would perhaps be fairer to
emphasize the comparative performance evaluation of the
four algorithms as the main contribution of this paper.}\label{intropar5}
    \item \todo[inline, color=green!30]{2. Related Work
   - While the authors do list several related
contributions, they do so while focused on (1) the
sensor(s) used, (2) the parameters of the state vector, and
(3) the type of filter used. This information could be
represented more compactly in a table.}\label{related1}
    \item \todo[inline, color=orange!30]{2. Related Work - Some comment
regarding the contributions and limitations of related work
would be appreciated. A few references (e.g. 31) are
missing from this section.}\label{related2}
\item \todo[inline, color=green!30]{3formula:  A. General model: the authors define the state vector
as the vehicle's three dimensional position. If orientation
measurements are assumed to be available, the authors
should consider making this assumption explicit.
}\label{formula1}
\item \todo[inline, color=orange!30]{3 formula: Linear/non-linear mixed motion model. The authors
introduce non-linearity by proposing a feedback model where
velocity is a function of the bathymetry at the estimated
position.  This appears somewhat contrived or of limited
applicability; as an alternative, the authors could instead
consider a different model (e.g. unicycle). This choice of
a model has no bearing on the next sections, as the
Methodology section describes general purpose filters - as
such, this particular model could be moved to the section
on experimental results.}\label{formula2}
\item \todo[inline, color=green!30]{3 formula: B. Model for MPF. The authors could consider moving
this to subsection IV.D, as this is a decomposition
necessitated by the use of the MPF. The notation, taken
from Schon's 2005 paper [28], is left unexplained for the
remainder of the paper (see later comments) }\label{formula3}
    \item \todo[inline, color=green!30]{4method:  the subsections on the two Kalman filter variants
(A.EKF,B.UKF) are somewhat lacking in details in comparison
with the following subsections on particle filters. A few
more remarks would be welcome (e.g. how is gridded
bathymetric data
used when computing the Jacobians? Are any local
approximations used?).
}\label{method1}
    \item \todo[inline, color=orange!30]{4 method: Like the subsections on the EKF and UKF, the
subsection on the Particle filter provides a description of
the filter, but only the equations to weight evaluation and
how to obtain the estimate from particles are shown}\label{method2}
    \item \todo[inline, color=green!30]{4 method: The subsection on the marginalized particle filter is
by far the most detailed of the four. While relevant, most
of the equations presented here are of limited use, as very
few of the terms are introduced or explained. The reader
must find Schon's 2005 paper (where most of equations 11
through 29 are taken from) to understand the meaning and
relevance of each of the terms. Moreover, given that these
pertain to the general linear/non-linear mixed model
("model 3" in the original paper), together with the space 
limitations of a conference submission, the authors should
consider simplifying and introducing these equations 
strictly as needed (instead of using the general versions),
or refer the reader to the relevant literature (e.g. the A
 matrix could be removed from the equations under the 
proposed mixed model, as the linear component is a single 
integrator, so A=I) }\label{method3}
    \item \todo[inline, color=green!30]{4 method: Finally, the authors could revise section IV to provide a more balanced overview of the four filters.}\label{method4}
    \item \todo[inline, color=green!30]{5 experiment: The authors state early on that 100 runs were conducted for each lake and filter combination - remarks on how these were aggregated to produce the results in figure 2 and tables 2 and 3 would be appreciated.}\label{exper1}
    \item \todo[inline, color=green!30]{5 experiment: in tables 2 and 3, listing the computation time (instead of simulation time) of each filter could make for a stronger comparative evaluation}\label{exper2}
    
    \item \todo[inline, color=green!30]{Style suggestions (very minor)
- Figure 2: Change RBPF to MPF in the figure legend for 
consistency with the text
- Figure 2: consider using figures in a vector format (e.g.
eps/pdf/svg) to avoid artifacts
- Place table captions above tables}\label{stylesugg}
    
     \item \todo[inline, color=red!30]{1 The source of real-time bathymetry data and the source of
motion measurement data in the simulation are not described
in the experimental section. Is it a replay simulation or a
simulation experiment using interpolation to get data?
2 In the conclusion section, the PF algorithm result is
better when the a water body has enough terrestrial
variations, but the definition of whether the water body
has enough terrestrial variations or not is not very clear.
It is recommended to introduce a variable related to the
complexity of the terrain and explain the threshold.
3 All simulation experiments did not mention the cost of
calculation.
}\label{secondcomment}

\item \todo[inline, color=green!30]{clear up Terrain Based Navigation (TBN)}\label{todotbn}

\item \todo[inline, color=green!30]{What is more different from what can be found elsewhere is
the Linear/Nonlinear mixed motion model of Equation (5),
but to which no explanation whatsoever is provided. It is
left to the reader to guess what is even the intuition
behind such model (it seems to be some sort of simple
linear LS squares approximation of the local floor
gradient).}\label{todotbn}

% \item \todo[inline, color=red!30]{}
% \item \todo[inline, color=red!30]{}
% \item \todo[inline, color=red!30]{}
% \item \todo[inline, color=red!30]{}





    
\end{enumerate}
